Efficiently Discovering Hammock Paths from Induced Similarity Networks

Similarity networks are important abstractions in many information management applications such as recommender systems, corpora analysis, and medical informatics. For instance, by inducing similarity networks between movies rated similarly by users, or between documents containing common terms, and or between clinical trials involving the same themes, we can aim to find the global structure of connectivities underlying the data, and use the network as a basis to make connections between seemingly disparate entities. In the above applications, composing similarities between objects of interest finds uses in serendipitous recommendation, in storytelling, and in clinical diagnosis, respectively. We present an algorithmic framework for traversing similarity paths using the notion of `hammock' paths which are generalization of traditional paths. Our framework is exploratory in nature so that, given starting and ending objects of interest, it explores candidate objects for path following, and heuristics to admissibly estimate the potential for paths to lead to a desired destination. We present three diverse applications: exploring movie similarities in the Netflix dataset, exploring abstract similarities across the PubMed corpus, and exploring description similarities in a database of clinical trials. Experimental results demonstrate the potential of our approach for unstructured knowledge discovery in similarity networks.

==> abs.tex <==
Similarity networks are important abstractions in many information
management applications such as recommender systems, corpora analysis,
and medical informatics. For instance, by inducing similarity networks
between movies rated similarly by users, or between documents containing
common terms, and or between clinical trials involving the same themes,
we can aim to find the global structure of connectivities underlying
the data, and use the network as a basis to make connections between
seemingly disparate entities. In the above applications, composing
similarities between objects of interest finds uses in serendipitous
recommendation, in storytelling, and in clinical diagnosis, respectively.
We present an algorithmic framework for traversing similarity paths
using the notion of `hammock' paths which are generalization of traditional
paths. Our framework is exploratory in nature so that, given starting
and ending objects of interest, it explores candidate objects for
path following, and heuristics to admissibly estimate the potential
for paths to lead to a desired destination. We present three diverse
applications: exploring movie similarities in the Netflix dataset,
exploring abstract similarities across the PubMed corpus, and exploring
description similarities in a database of clinical trials. Experimental
results demonstrate the potential of our approach for unstructured
knowledge discovery in similarity networks.

